Delicate Textured Mesh Recovery from NeRF via Adaptive Surface Refinement

Neural Radiance Fields (NeRF) have constituted a remarkable breakthrough in image-based 3D reconstruction. However, their implicit volumetric representations differ significantly from the widely-adopted polygonal meshes and lack support from common 3D software and hardware, making their rendering and manipulation inefficient. To overcome this limitation, we present a novel framework that generates textured surface meshes from images. Our approach begins by efficiently initializing the geometry and view-dependency decomposed appearance with a NeRF. Subsequently, a coarse mesh is extracted, and an iterative surface refining algorithm is developed to adaptively adjust both vertex positions and face density based on re-projected rendering errors. We jointly refine the appearance with geometry and bake it into texture images for real-time rendering. Extensive experiments demonstrate that our method achieves superior mesh quality and competitive rendering quality.

==> tabs/storage_360.tex <==
\begin{table*}[!t]
\begin{center}

\begin{tabular}{lcccc}
\hline
& Garden & Bicycle & Stump & Mean \\
\hline
MobileNeRF~\cite{chen2022mobilenerf}    & 239.00 & 400.00 & 337.00 & 325.33  \\
Ours                                    & 188.94 & 180.52 & 191.06 & 186.84 \\
\hline
\end{tabular}

\end{center}
\caption{
Disk storage (MB) on the Mip-NeRF 360 dataset.
}
\label{table:storage_360}
\end{table*}



==> tabs/storage_llff.tex <==
\begin{table*}[!t]
\begin{center}

\begin{tabular}{lccccccccc}
\hline
& Room & Fern & Leaves & Fortress & Orchids & Flower & Trex & Horns & Mean \\
\hline
SNeRG~\cite{hedman2021snerg}            & 149.00 & 288.00 & 408.00 & 162.00 & 704.00 & 321.00 & 251.00 & 415.00 & 337.25 \\
MobileNeRF~\cite{chen2022mobilenerf}    & 127.00 & 147.00 & 353.00 & 89.00 & 372.00 & 151.00 & 162.00 & 211.00 & 201.50 \\
Ours                                    & 139.12 & 123.53 & 131.62 & 133.09 & 138.93 & 155.28 & 86.78 & 90.36 & 124.84 \\
\hline
\end{tabular}

\end{center}
\caption{
Disk storage (MB) on the LLFF dataset.
}
\label{table:storage_llff}
\end{table*}



==> tabs/storage_syn.tex <==
\begin{table*}[!t]
\begin{center}

\begin{tabular}{lccccccccc}
\hline
& Chair & Drums & Ficus & Hotdog & Lego & Materials & Mic & Ship & Mean \\
\hline
SNeRG~\cite{hedman2021snerg}            & 141.00 & 44.00 & 43.00 & 67.00 & 114.00 & 134.00 & 22.00 & 129.00 & 86.75 \\
MobileNeRF~\cite{chen2022mobilenerf}    & 107.00 & 120.00 & 80.00 & 88.00 & 199.00 & 191.00 & 50.00 & 171.00 & 125.75 \\
Ours                                    & 59.27 & 81.87 & 79.81 & 90.59 & 68.77 & 82.14 & 55.17 & 70.63 & 73.53 \\
\hline
\end{tabular}

\end{center}
\caption{
Disk storage (MB) on the NeRF-synthetic dataset.
}
\label{table:storage_syn}
\end{table*}


